Selftok: Discrete Visual Tokens of Autoregression, by Diffusion, and for Reasoning

We completely discard the conventional spatial prior in image representation and introduce a novel discrete visual tokenizer: Self-consistency Tokenizer (Selftok). At its design core, we compose an autoregressive (AR) prior -- mirroring the causal structure of language -- into visual tokens by using the reverse diffusion process of image generation. The AR property makes Selftok fundamentally distinct from traditional spatial tokens in the following two key ways: - Selftok offers an elegant and minimalist approach to unify diffusion and AR for vision-language models (VLMs): By representing images with Selftok tokens, we can train a VLM using a purely discrete autoregressive architecture -- like that in LLMs -- without requiring additional modules or training objectives. - We theoretically show that the AR prior satisfies the Bellman equation, whereas the spatial prior does not. Therefore, Selftok supports reinforcement learning (RL) for visual generation with effectiveness comparable to that achieved in LLMs. Besides the AR property, Selftok is also a SoTA tokenizer that achieves a favorable trade-off between high-quality reconstruction and compression rate. We use Selftok to build a pure AR VLM for both visual comprehension and generation tasks. Impressively, without using any text-image training pairs, a simple policy gradient RL working in the visual tokens can significantly boost the visual generation benchmark, surpassing all the existing models by a large margin. Therefore, we believe that Selftok effectively addresses the long-standing challenge that visual tokens cannot support effective RL. When combined with the well-established strengths of RL in LLMs, this brings us one step closer to realizing a truly multimodal LLM. Project Page: https://selftok-team.github.io/report/.

==> figures/fig3.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-11mm}
\includegraphics[width=\linewidth]{example-image-b}
    \caption{The AR training loss using spatial tokens does not degrade under different token sequence perturbations, unlike language or Selftok tokens with AR property.}
    \label{fig:3}
\vspace{-3mm}
\end{wrapfigure}

==> figures/fig5.tex <==
\begin{figure*}[!htb]
    \centering
    \footnotesize
    % \begin{subfigure}{\textwidth}
         \includegraphics[width=\textwidth]{figures/AR_Figure_crop.pdf}
         % \phantomcaption
         % \label{fig:5a}
    % \end{subfigure}
    \caption{Illustration of the proposed data format for cross-modality and cross-task alignment.}
    \vspace*{-3mm}
    \label{fig:ar}
\end{figure*}

==> figures/fig7.tex <==
\begin{figure*}
    \centering
    \footnotesize
    \begin{subfigure}[t]{0.45\textwidth}
         \includegraphics[width=0.9\textwidth]{example-image-b}
         \phantomcaption
         \label{fig:7a}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth} 
         \includegraphics[width=0.9\textwidth]{example-image-b}
         \phantomcaption
         \label{fig:7b}   
    \end{subfigure}
    %\vspace*{-3mm}
    \caption{Disentanglement}
    \vspace*{-3mm}
    \label{fig:disentangle}
\end{figure*}

==> figures/fig8.tex <==
\begin{wrapfigure}{r}{0.35\textwidth}
\vspace{-5mm}
\footnotesize
\includegraphics[width=\linewidth]{figures/figure8.pdf}
\vspace{-5mm}
\caption{\justifying The recursive Bellman equation fails when a child node $v_{l}$ (\ie, future token) anti-causally affects a parent node $v_{k+1}$.}
\label{fig:8}
\vspace{-5mm}
\end{wrapfigure}

==> figures/fig_interpolation.tex <==
\begin{figure*}
    \centering
    \footnotesize
    \includegraphics[width=\textwidth]{./figures/interpolation.pdf}
    \vspace*{-5mm}
    \caption{Interpolation of tokens from two images.[ToDo] Interpolation of tokens from two images.[ToDo] Interpolation of tokens from two images.[ToDo] Interpolation of tokens from two images.[ToDo]}
    \vspace*{-1mm}
    \label{fig:interpolation}
\end{figure*}

==> figures/fig_rl_ab.tex <==
\begin{wrapfigure}{r}{0.35\textwidth}
\vspace{-10mm}
\footnotesize
\includegraphics[width=\linewidth]{example-image-b}
\vspace{-2mm}
\caption{\justifying The qualitative ablation experiment results of visual RL.}
\label{fig:ab_rl}
\vspace{-5mm}
\end{wrapfigure}

==> tables/chateval.tex <==
\begin{table}[h]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{1.9pt}
    \begin{tabular}{@{}c l | c  c  c | c c |c c@{}}
    \toprule
    & \multirow{2}{*}{\centering \textbf{Benchmark {\tiny (Metric)}}}  & \textbf{Claude-3.5-}  & \textbf{GPT-4o}& \textbf{DeepSeek} & \textbf{OpenAI} & \textbf{OpenAI} & \textbf{DeepSeek}\\
    & & \textbf{Sonnet-1022}  & \textbf{0513} & \textbf{V3} & \textbf{o1-mini}& \textbf{o1-1217} &\textbf{R1} \\
    \midrule
    & Architecture &-&- & MoE &-&-& MoE \\
    & \# Activated Params& -&-& 37B&-&- & 37B \\
    & \# Total Params &-&-& 671B&-&- & 671B \\
    \midrule
    \multirow{10}{*}{English}& MMLU {\tiny (Pass@1)} & 88.3&87.2 & 88.5 & 85.2 & \textbf{91.8} & 90.8\\
     & MMLU-Redux {\tiny (EM)}& 88.9& 88.0 & 89.1 & 86.7&- & \textbf{92.9} \\
    & MMLU-Pro {\tiny (EM)}  & 78.0 & 72.6 & 75.9 & 80.3 &-& \textbf{84.0} \\
    & DROP {\tiny (3-shot F1)}  & 88.3 & 83.7 & 91.6 & 83.9 & 90.2 & \textbf{92.2}\\
    & IF-Eval {\tiny (Prompt Strict)}  & \textbf{86.5} & 84.3 & 86.1 & 84.8&- & 83.3 \\
    & GPQA Diamond {\tiny (Pass@1)}& 65.0 & 49.9 & 59.1 & 60.0 & \textbf{75.7} & 71.5&  \\
    & SimpleQA {\tiny (Correct)} & 28.4 & 38.2& 24.9 & 7.0 & \textbf{47.0} & 30.1 \\
     & FRAMES {\tiny (Acc.)}  & 72.5 & 80.5 & 73.3 & 76.9 & -&\textbf{82.5}\\
      & AlpacaEval2.0 {\tiny (LC-winrate)}  & 52.0 &  51.1 & 70.0 & 57.8 & - & \textbf{87.6}\\
       & ArenaHard {\tiny (GPT-4-1106)}  & 85.2 & 80.4 & 85.5 & 92.0 & - & \textbf{92.3}\\
    \midrule
    \multirow{4}{*}{Code} & LiveCodeBench {\tiny (Pass@1-COT)} & 38.9 & 32.9 & 36.2 & 53.8 & 63.4 & \textbf{65.9} \\
    & Codeforces {\tiny (Percentile)}& 20.3 & 23.6 & 58.7 & 93.4 & \textbf{96.6} & 96.3 \\
    & Codeforces {\tiny (Rating)}& 717 & 759 & 1134 & 1820 & \textbf{2061} & 2029 \\
    & SWE Verified {\tiny (Resolved)} & \textbf{50.8}&38.8&42.0 & 41.6 & 48.9 & 49.2\\
    & Aider-Polyglot {\tiny (Acc.)} & 45.3&16.0& 49.6 & 32.9 & \textbf{61.7}&53.3\\
    \midrule
    \multirow{3}{*}{Math} & AIME 2024 {\tiny (Pass@1)}  & 16.0 & 9.3 & 39.2 & 63.6 & 79.2 & \textbf{79.8} \\
    & MATH-500 {\tiny (Pass@1)} &78.3 & 74.6&90.2 & 90.0 & 96.4 & \textbf{97.3} \\
    & CNMO 2024 {\tiny (Pass@1)} & 13.1 & 10.8 &43.2 & 67.6 & - & \textbf{78.8} \\
    \midrule
    \multirow{3}{*}{Chinese} & CLUEWSC {\tiny (EM)}&  85.4 & 87.9 & 90.9 & 89.9 & - &\textbf{92.8}\\
    & C-Eval {\tiny (EM)} & 76.7 & 76.0 & 86.5 & 68.9 & - & \textbf{91.8}\\
     & C-SimpleQA {\tiny (Correct)}  & 55.4 & 58.7 & \textbf{68.0} & 40.3 & -& 63.7 \\
    \bottomrule
    \end{tabular}
    \caption{ Comparison between \dsri{} and other representative models. 
    }
    \label{tab:main}
\end{table}


==> tables/distill_eval.tex <==
\begin{table}[h]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}l *{6}{c} @{}}
    \toprule
    \multirow{3}{*}{\centering\textbf{Model}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{AIME 2024}}} & \multirow{2}{*}{\textbf{MATH-500}} & \textbf{GPQA} & \textbf{LiveCode} & \multirow{2}{*}{\textbf{CodeForces}} \\
    &  &  &  & \textbf{Diamond} & \textbf{Bench} \\
    \cmidrule(lr){2-3}
     & pass@1 & cons@64 & pass@1 & pass@1 & pass@1 & rating \\
    \midrule
    \textbf{GPT-4o-0513} & 9.3 & 13.4 & 74.6  & 49.9 & 32.9 &  759\\
    \textbf{Claude-3.5-Sonnet-1022} & 16.0 & 26.7 & 78.3  & 65.0 & 38.9 &  717\\
    \textbf{OpenAI-o1-mini} & 63.6 & 80.0 & 90.0 &  60.0 & 53.8 &  \textbf{1820}\\
    \textbf{QwQ-32B-Preview} & 50.0 & 60.0 & 90.6 & 54.5 & 41.9 &  1316 \\
    \midrule
    \textbf{DeepSeek-R1-Distill-Qwen-1.5B} & 28.9 & 52.7 & 83.9 & 33.8 & 16.9 & 954 \\
    \textbf{DeepSeek-R1-Distill-Qwen-7B} & 55.5 & 83.3 & 92.8 & 49.1 & 37.6 & 1189 \\
    \textbf{DeepSeek-R1-Distill-Qwen-14B} & 69.7 & 80.0 & 93.9 &  59.1 & 53.1 & 1481 \\
    \textbf{DeepSeek-R1-Distill-Qwen-32B} & \textbf{72.6} & {83.3} & {94.3} & {62.1} & {57.2} & 1691 \\
    \textbf{DeepSeek-R1-Distill-Llama-8B} & 50.4 & 80.0 & 89.1 & 49.0 & 39.6 & 1205 \\
    \textbf{DeepSeek-R1-Distill-Llama-70B} & 70.0 & \textbf{86.7} & \textbf{94.5} & \textbf{65.2} & \textbf{57.5} & 1633 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Comparison of DeepSeek-R1 distilled models and other comparable models on reasoning-related benchmarks.}
    \label{tab:distill}
\end{table}



==> tables/distill_vs_rl.tex <==
\begin{table}[h]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}l *{6}{c} @{}}
    \toprule
    \multirow{3}{*}{\centering\textbf{Model}} & \multicolumn{2}{c}{\textbf{AIME 2024}} & \textbf{MATH-500} & \textbf{GPQA Diamond} & \textbf{LiveCodeBench}  \\

    \cmidrule(lr){2-3}
     & pass@1 & cons@64 & pass@1& pass@1 & pass@1 \\
    \midrule
    \textbf{QwQ-32B-Preview} & 50.0 & 60.0 & 90.6 & 54.5 & 41.9  \\
    \textbf{DeepSeek-R1-Zero-Qwen-32B} & 47.0 & 60.0 & 91.6  & 55.0 & 40.2  \\
    \textbf{DeepSeek-R1-Distill-Qwen-32B} & \bf{72.6} & \bf{83.3} & \bf{94.3}  & \bf{62.1} & \bf{57.2}\\
    \bottomrule
    \end{tabular}
    }
    \caption{\centering Comparison of distilled and RL Models on Reasoning-Related Benchmarks.}
    \label{tab:distill_vs_rl}
\end{table}

